Global Convergence and Stability of Stochastic Gradient Descent

In machine learning, stochastic gradient descent (SGD) is widely deployed to train models using highly non-convex objectives with equally complex noise models. Unfortunately, SGD theory often makes restrictive assumptions that fail to capture the non-convexity of real problems, and almost entirely ignore the complex noise models that exist in practice. In this work, we make substantial progress on this shortcoming. First, we establish that SGD's iterates will either globally converge to a stationary point or diverge under nearly arbitrary nonconvexity and noise models. Under a slightly more restrictive assumption on the joint behavior of the non-convexity and noise model that generalizes current assumptions in the literature, we show that the objective function cannot diverge, even if the iterates diverge. As a consequence of our results, SGD can be applied to a greater range of stochastic optimization problems with confidence about its global convergence behavior and stability.

==> section/notation.tex <==
We refer to the objective function of the stochastic optimization problem by $F(\theta)$, and its gradient evaluated at $\theta$ by $\dot F(\theta)$. We let $f(\theta,X)$ denote the stochastic objective function that is used to generate $F$, by taking an expectation over $X$, the random variable. We denote the derivative of $f$ with respect to its first argument and evaluated at $(\theta,X)$ by $\dot f(\theta,X)$. We let $\lbrace X_k \rbrace$ denote independent copies of $X$, and let $\mathcal{F}_k$ denote the $\sigma$-algebra generated by $\lbrace X_1,X_2,\ldots,X_k \rbrace$.

==> section/spurious-continuous-gd.tex <==
In \cref{theorem-global-convergence}, we prove that SGD's iterates (including Gradient Descent's iterates) \textit{either} diverge or they must converge to a stationary point; in particular, our result excludes the possibility of convergence to a limit cycle. However, in the continuous-time analysis of GD, for the objective function
\begin{equation}
F(\theta) = \begin{cases}
\exp\left( \frac{1}{\theta_1^2 - 1}  \right) & \theta_1 < 1 \\
0 & \theta_1 = 1 \\
-\exp\left( \frac{-1}{\theta_1^2 - 1} \right) \sin\left( \frac{1}{\theta_1 - 1} - \theta_2  \right) & \theta_1 > 1,
\end{cases}
\end{equation}
there exist an initialization for continuous-time GD (i.e., that solves $\frac{d\theta}{dt} = - \dot F(\theta)$) such that the trajectory of continuous-time GD approaches the limit cycle of $\theta_1 = 1$, where we interpret $\theta$ to be in polar coordinates with $\theta_1$ representing the radius and $\theta_2$ representing the angle (this example is a slight modification of \citep[Example 3]{palis2012}).

At first glance, this dissonance can be dismissed as the consequence of discretization, which is well-known to produce spurious solutions \citep{stuart1994}; however, there is a substantial body of work that uses continuous-time GD to analyze GD and SGD \citep{chizat2018,du2018,mei2018,rotskoff2018,lee2019,mertikopoulos2020,sirignano2020,sirignano2020mean,sirignano2022}. Moreover, this body of work relies on the following intuition: 
\begin{quote}
``It is natural to expect that, owing to the fact that [the learning rate] is small, the noise washes out and that the asymptotic behavior
of [SGD] is closely related to the asymptotic behavior of the ODE.'' \citep[Pg. 3]{benaim1999}.
\end{quote}

Based on this intuition, we should expect SGD or GD to be able to converge to a limit cycle for the above example given that continuous-time GD converges to this limit cycle, which is explicitly not allowed by \cref{theorem-global-convergence}. To address this controversy, we prove directly for the above example that the limit cycle of continuous-time GD is a spurious solution for GD with diminishing step size. The details are provided in

\begin{theorem}
Let $\theta = (\theta_1,\theta_2)$ be any point with $\theta_1 \geq 0$ and $\theta_2 \in \mathbb{R}$ such that the trajectory of $\frac{d\theta}{dt} = - \dot F(\theta)$ with this initial value has the limit cycle of $\theta_1 = 1$. Then for any non-negative sequence of step sizes, $\lbrace \alpha_k: k+1 \in \mathbb{N} \rbrace$, satisfying $\sum_{k} \alpha_k = \infty$ and $\sum_k \alpha_k^2 < \infty$, the sequence $\lbrace \phi_k : k+1 \in \mathbb{N} \rbrace$, defined by $\phi_0 = \theta$ and $\phi_{k+1} = \phi_k - \alpha_k \dot F(\phi_k)$, will either converge to a single point or diverge.
\end{theorem}



%Unfortunately, the existence of spurious solutions for continuous gradient methods calls into question the \textit{general applicability}\footnote{By this we mean that there must be very strict assumptions (and likely unrealistic) on the network or the initialization (e.g., Theorem 3.3 of \cite{chizat2018}) for the continuous gradient method to be well-approximated by a (stochastic) gradient method. And, without satisfying such assumptions, these analyses cannot be used as guidance for how the training and learning of neural networks occurs.} of a number of well-cited and influential analyses on understanding deep learning that rely on continuous gradient techniques \citep{chizat2018,du2018,mei2018,rotskoff2018,lee2019,sirignano2020,sirignano2020mean,sirignano2022}.
